HPC Storage Service Autotuning Using Variational-Autoencoder-Guided Asynchronous Bayesian Optimization

Distributed data storage services tailored to specific applications have grown popular in the high-performance computing (HPC) community as a way to address I/O and storage challenges. These services offer a variety of specific interfaces, semantics, and data representations. They also expose many tuning parameters, making it difficult for their users to find the best configuration for a given workload and platform. To address this issue, we develop a novel variational-autoencoder-guided asynchronous Bayesian optimization method to tune HPC storage service parameters. Our approach uses transfer learning to leverage prior tuning results and use a dynamically updated surrogate model to explore the large parameter search space in a systematic way. We implement our approach within the DeepHyper open-source framework, and apply it to the autotuning of a high-energy physics workflow on Argonne's Theta supercomputer. We show that our transfer-learning approach enables a more than $40\times$ search speedup over random search, compared with a $2.5\times$ to $10\times$ speedup when not using transfer learning. Additionally, we show that our approach is on par with state-of-the-art autotuning frameworks in speed and outperforms them in resource utilization and parallelization capabilities.

==> sections/Discussion.tex <==
%Having run so many experiments and evaluated so many configurations of the HEP workflow, two questions arise. First, can we measure the relative influence of each parameter on the workflow run time? Second, can we better understand why certain configurations perform well while some perform poorly? This section addresses these two questions.

%\subsection{Relative effect of individual parameters}
%\label{sec:Discussion:effect}

%\note{TODO: Romain. Here we probably need an experiment that samples a bunch of configuration (4-node, full-workflow, 19 parameters) and explain the maths that leads to computing the feature importance.}

%\subsection{Understanding HEPnOS performance and optimizing further}
%\label{sec:Discussion:profiling}

The Mochi developers implemented profiling tools to help understand the root cause of performance degradation. These tools are included in the Margo library and can be enabled to track metrics related to networking the threads usage. These tools were actually used in the past to manually tune HEPnOS and the workflow we used in this paper~\cite{Ramesh2021Symbiosys}.

We reused the same methodology here to take the best-performing and poorly-performing configurations from Section~\ref{sec:Experiments:fullwflow} and understand what differs inside HEPnOS that makes it perform better or worse.

Figure~\ref{fig:Discussion:unbalance} shows the normalized number of RPCs received by each key/value storage provider in HEPnOS, when using the best-performing configuration. We can see an important load imbalance across servers. Solving this imbalance by changing the way HEPnOS distributes data across database instances could further improve performance. This change is not yet something configurable via Bedrock.

Figure~\ref{fig:Discussion:cumulative} shows the cumulative time spent servicing RPCs in servers with the best and worst configuration, and Figure~\ref{fig:Discussion:relative} details the relative amount of time spent in different parts of the code. We can see that an important part of the execution time is spent in memory registration for RDMA operations, especially for the worst-performing configuration because of its small batch size. In both cases, this overhead could be eliminated by integrating a pool of pre-registered memory buffers into HEPnOS servers. %\PB{Why analyse the worst config? Why not default or previous best?}

\begin{figure*}[t!]
    \begin{subfigure}[t]{5.6cm}
        \includegraphics[width=5.6cm]{img/discussion/FAST_dataloader_best_configuration_call_counts.pdf}
        \caption{Normalized RPC count per provider (sorted by RPC count) in the best-performing configuration.}
        \label{fig:Discussion:unbalance}
    \end{subfigure}
    \quad
    \begin{subfigure}[t]{5.6cm}
        \includegraphics[width=5.6cm]{img/discussion/FAST_dataloader_cumulative_execution_time.pdf}
        \caption{Cumulative RPC execution time in servers in the best and worst configurations.}
        \label{fig:Discussion:cumulative}
    \end{subfigure}
    \quad
    \begin{subfigure}[t]{5.6cm}
        \includegraphics[width=5.6cm]{img/discussion/FAST_dataloader_relative_contributions.pdf}
        \caption{Relative time spent in different sections of the server's RPC handler code in the best and worst configuration.}
        \label{fig:Discussion:relative}
    \end{subfigure}
    \caption{Execution information obtained from internal profiling and manual analysis.}
    \label{fig:Discussion:profiling}
\end{figure*}

These results show that while DeepHyper can do a great deal of optimization automatically for the user, coupling it with subsequent human analysis of profiling data can help further improve the design of the workflow and storage system.

==> sections/old/Evaluation.tex <==
In this section, we evaluate the effectiveness of our TL-enabled autotuning workflow.

\subsection{Platform and configurations}

The experiments presented in this paper were carried out on the Cray XC40 ``MachineA'' supercomputer. %~\cite{Theta}.
MachineA is an 11.7-petaflops supercomputer composed of 4,392 nodes, each featuring a 64-core, 1.3-GHz Intel Xeon Phi 7230 processor, and interconnected via a Cray Aries network with a Dragonfly topology.

We implemented PABO within the asynchronous BO of DeepHyper, a scalable open source package that was originally developed for hyperparameter optimization of machine learning methods. 
For PABO, for each parameter integer and real parameter $x_j$, we set $\sigma_j = max(1.0, (u_j - l_j) / 10.0)$; for each of the categorical parameter, we set a weight value of 8.0 for the best and 1.0 for other values; the normalized vector of weights is then given as a probability vector for the multinoulli distribution. The surrogate model used is a random forest regressor with \PB{how many trees}. \PB{the $\kappa$ value in BO?}  
Each experiment is deployed on 128 nodes that DeepHyper uses to execute a number of HEP workflow instances. Unless specified otherwise, each workflow instance uses 4 nodes. 1 node is reserved for HEPnOS. The remaining 3 nodes execute the dataloader and the PEP application consecutively. This lets DeepHyper run with 32 workers that evaluate up to 32 configurations in parallel. In Section~\ref{sec:Experiments:scaleup} we scale the HEP workflow to 8 nodes (2 HEPnOS nodes, 6 application nodes) and 16 nodes (4 HEPnOS nodes, 12 application nodes). The FermiLab team kindly provided us with a sample of 200 HDF5 files (totalling 26.5 GiB), which also limits the scale at which we can run our experiments. We use 50 files for 4-node experiments, 100 files for 8 nodes, and 200 files for 16 nodes.

Initial executions of the HEP workflow on 4 nodes with manually selected parameters led to a run time in the order of 90 seconds for the dataloader, and 90 seconds for the PEP application. Hence, to prevent a bad configuration from taking too long to complete, which would prevent DeepHyper from evaluating other, potentially better configurations, we limit the execution time of each workflow instance to 600 seconds (300 seconds per step). If a workflow step (dataloader or PEP) hasn't completed within its time limit, it is killed, and the evaluation returns a run time of $\infty$.

\subsection{Parameter space and evaluation metrics}

Although an arbitrarily large number of parameters could be considered thanks to HEPnOS' use of Bedrock, we limit the present study to the 19 parameters listed in Table~\ref{tab:parameters}. These parameters are the first parameters one would seek to optimize for this type of workflow. They affect multiple levels of the workflow, from the launcher command (e.g., the mapping of processes to physical nodes), to optimizations in each component (e.g, various batch sizes), the structure of the storage system (e.g., its number of databases and mapping of threads to databases), down to the network layer (e.g., whether to use busy-spinning or blocking on \emph{epoll}). This parameter space contains $6\times 10^{22}$ distinct configurations.

In the following, to avoid confusion, we call \emph{run time} the execution time of an HEP workflow instance (this run time is the objective DeepHyper/PABO aims to minimize), and use the letter $t$ to represent such a run time. We call \emph{search time} the execution time of the DeepHyper/PABO workflow, and use the letter $\tau$ to represent it.
We use two metrics to evaluate the advantage of TL.

    \paragraph{Search speedup:} By executing a search with and without TL, we can show how much faster it converges towards equally-performing configurations. Let $t$ be a target run time, and $T(t)$ and $T'(t)$ be the minimum amount of search time required by DeepHyper/PABO to find a configuration of the HEP workflow with an run time under $t$, respectively without and with TL. %Let $t_{min}^{noTL}$ and $t_{min}^{TL}$ be the run-time of the best-performing configuration found without and with TL respectively, and $t_{min} = max(t_{min}^{noTL}, t_{min}^{TL})$. We define the \emph{final-configuration speedup} as follows.
    %\[ S_{final} = \frac{T(t_{min})}{T'(t_{min})} \]
    %Unless the parameter space has been searched exhaustively, $S_{final}$ has little meaning beyond representing the speedup associated with the best configuration at the time we decide to stop the search. A more relevant metric is the \emph{expected search speedup}, defined as follows.
    We define the \emph{expected search speedup} as
    \[ E[S] = \frac{1}{t_{first} - t_{min}} \int_{t=t_{min}}^{t_{first}} \frac{T(t)}{T'(t)} dt, \]
    where $t_{first}$ is the run time of the first configuration evaluated and $t_{min}$ is the best run-time found either with or without TL, whichever is largest (otherwise one of either $T(t_{min})$ or $T'(t_{min})$ is unknown).

    \paragraph{Improvement factor:} Let $\tau$ represent the search time of the DeepHyper/PABO workflow. Let $R(\tau)$ and $R'(\tau)$ be the run time of the best-performing configuration found by DeepHyper/PABO over the search-time $\tau$ respectively without and with TL. We define the \emph{improvement factor} as
    \[ F(\tau) = \frac{R(\tau)}{R'(\tau)} \]
    and the expected improvement factor as
    \[ E[F] = \frac{1}{D} \int_{\tau=0}^{D} \frac{R(\tau)}{R'(\tau)} d\tau \]
    where $D$ is the full duration considered (1 hour in our experiments).
    The improvement factor represents how much better the configuration found using TL is, within a given search time, compared with the configuration found without TL within the same search time. The expected improvement factor represents what improvement factor we can expect on average when running DeepHyper/PABO for a duration drawn uniformly within a range $[0, D]$.\footnote{Note that as $D \rightarrow +\infty$ we should expect $E[F] \rightarrow 1$ since with no search time limit, DeepHyper/PABO would exhaustively evaluate all configurations and find the same optimal one regardless of whether it used TL to begin with.}

We further average these metrics over several runs for each experiment. Because each experiment requires a significant amount of resources however, we limit each experiment to 5 repetitions.

\begin{sidewaystable}\small
\centering
\begin{tabular}{l|l|l|l|l|}
\cline{2-5}
 & \textbf{Parameter} & \textbf{Range} & \textbf{Distribution} & \textbf{Description} \\ \hline
\multicolumn{1}{|l|}{\textbf{Common}} & BusySpin & True/False & Uniform & Whether Mercury should busy-spin instead of blocking on epoll \\ \hline
\multicolumn{1}{|l|}{\multirow{7}{*}{\textbf{HEPnOS}}} & ProgressThread & True/False & Uniform & Whether to use a dedicated network progress thread in HEPnOS servers \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & NumRPCthreads & {[}0, 63{]} & Uniform & Number of threads used by HEPnOs servers to service RPC \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & NumEventDBs & {[}1, 16{]} & Uniform & Number of database instances per HEPnOS server for Events \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & NumProductDBs & {[}1, 16{]} & Uniform & Number of database instances per HEPnOS server for Products \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & NumProviders & {[}1, 32{]} & Uniform & Number of database providers per HEPnOS server \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & ThreadPoolType & \{fifo, fifo\_wait, prio\_wait\} & Uniform & Argobots thread pool type each provider uses \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & PESperNode & \{1, 2, 4, 8, 16, 32\} & Uniform & Number of HEPnOS server processes per physical node \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Dataloader}}} & ProgressThread & True/False & Uniform & Whether to use a dedicated network progress thread in Dataloader processes \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & WriteBatchSize & {[}1, 2048{]} & Log-uniform & Size of the batches (in number of events used when sending data to HEPnOS \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & PESperNode & \{1, 2, 4, 8, 16, 32\} & Uniform & Number of Dataloader processes per physical node \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{\textbf{PEP}}} & ProgressThread & True/False & Uniform & Whether to use a dedicated network progress thread in PEP processes \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & NumThreads & {[}1, 31{]} & Uniform & Number of threads use to process data in parallel \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & InputBatchSize & {[}8, 1024{]} & Log-uniform & Batch size (in number of events) to use when loading data from HEPnOS \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & OuputBatchSize & {[}8, 1024{]} & Log-uniform & Batch size (in number of events) to use when sending data across PEP processes \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & PESperNode & \{1, 2, 4, 8, 16, 32\} & Uniform & Number of PEP processes per physical node \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Dataloader\\ (cont'd)\end{tabular}}}} & LoaderAsync & True/False & Uniform & Use threads to asynchronously send batches to HEPnOS \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & LoaderAsyncThreads & {[}1, 63{]} & Log-uniform & Number of threads for asynchronous store in Dataloader \\ \hline
\multicolumn{1}{|l|}{\textbf{PEP (cont'd)}} & UsePreloading & True/False & Uniform & Use batch-prefetching of data products instead of per-product load \\ \hline
\end{tabular}
\caption{List of parameters making up the parameter space explored in this work.}
\label{tab:parameters}
\end{sidewaystable}

In all the figures, orange refers to results obtained without any TL, while blue refers to results obtained with TL. Labels are shown in the form of three numbers $x, y, z$, where $x$ is the number of steps of the HEP workflow (1 or 2), $y$ is the number of parameters of the parameter space, and $z$ is the number of nodes per HEP workflow instance. This label is followed by $TL$ for results that used transfer-learning.

\subsection{Preliminary experiments}
\label{sec:Experiments:preliminary}

%\note{NOTE: we might want to do more preliminary experiments, for instance sampling configurations and running them to evaluate the variability in run-time and its range.}

Before diving into experiments involving TL, we first run the DeepHyper/PABO workflow once to obtain a baseline to transfer from. We run only the first step of the workflow (dataloader), using 4-node instances and 50 input HDF5 files, with DeepHyper/PABO using 128 nodes in total. %Each experiment is reproduced 5 times with different seeds.
The parameter space consists of the first 11 parameters listed in Table~\ref{tab:parameters}.

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{img/preliminary/plot_scatter_multi.pdf}
        \caption{Run-time of single-step workflow instances evaluated by DeepHyper/PABO as the search workflow progresses.}
        \label{fig:Experiments:preliminary:a}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{img/preliminary/plot_objective_multi.pdf}
        \caption{Run-time of the corresponding best-performing configuration as a function of the search time.}
        \label{fig:Experiments:preliminary:b}
    \end{subfigure}
    \caption{Preliminary experiment: DeepHyper/PABO workflow using 128 nodes, each HEP workflow instance uses 4 nodes. The HEP workflow only consists of the dataloader.}
    \label{fig:Experiments:preliminary}
\end{figure}

Figure~\ref{fig:Experiments:preliminary:a} shows the run time of each workflow instance evaluated by DeepHyper/PABO as the parameter-space exploration progress. At the beginning of the search, the run times are scattered as DeepHyper/PABO samples the parameter space uniformly. As BO kicks in, it then concentrates the search towards regions of the parameter space that lead to good performance, to improve on known well-performing configurations.

Figure~\ref{fig:Experiments:preliminary:b} shows the average run-time of the best-performing configuration and the minimum and maximum across the five repetitions of the DeepHyper/PABO workflow. As DeepHyper/PABO runs 32 instances in parallel, with configurations uniformly sampled across the parameter space, and as each instance requires 10 to 100 seconds to run, it only takes a few minutes for the minimum run-time to converge.

This experiment shows that the performance of the dataloader can vary widely depending on its configuration and the configuration of HEPnOS. The default parameters initially used for this workflow, which originally led to a 90-second run time, was easily outperformed by DeepHyper/PABO, which found configurations completing in as little as 9 seconds (a $10\times$ speedup). In fact, 9 seconds appears to be a hard-limit for this dataloader application, and stems from maximizing the hardware usage (network, memory, CPUs, and storage). We noted that a number of configurations achieved this run time. These configurations often differed in parameters such as the number of threads, which could be increased without negatively impacting the run time, but without improving resource utilization either.

\subsection{From a single step to the full workflow}
\label{sec:Experiments:fullwflow}

We now consider the full HEP workflow (dataloader + PEP). % on 4 nodes per instance, using 50 input files.
The parameter space consists of the first 16 entries in Table~\ref{tab:parameters}. We run the experiment with and without leveraging the knowledge obtained from the first of the five runs done in Section~\ref{sec:Experiments:preliminary}.

This scenario corresponds to the situation where, after having optimized a particular workflow, the user wants to add extra steps to it and has to find a good configuration for the new workflow.

%%%%%%%% 2-plot version of figure + corresponding text %%%%%%%% 
\begin{comment}
\begin{figure}[t]
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/single-to-full/plot_scatter_multi.pdf}
        \caption{Run-time of full workflow instances evaluated by DeepHyper/PABO as the search workflow progresses.}
        \label{fig:Experiments:fullwflow:a}
    \end{subfigure}
    \par\bigskip
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/single-to-full/plot_objective_multi.pdf}
        \caption{Run-time of the corresponding best-performing configurations as a function of the search time.}
        \label{fig:Experiments:fullwflow:b}
    \end{subfigure}
    \caption{Adding a workflow step: DeepHyper/PABO workflow uses 128 nodes, each HEP workflow instance uses 4 nodes. The HEP workflow consists of both dataloader and PEP application. We compare the executions with and without TL from results obtained in Section~\ref{sec:Experiments:preliminary}.}
    \label{fig:Experiments:fullwflow}
\end{figure}

Figure~\ref{fig:Experiments:fullwflow:a} shows that using TL allows DeepHyper/PABO to start from configurations that are generally better than without TL. This gives an advantage to the TL experiments very early on as instances are able to complete faster, leading to more evaluations, hence better configurations found.

Figure~\ref{fig:Experiments:fullwflow:b} shows the average run-time of the corresponding best-performing instances as the search progresses, and the corresponding minimum and maximum. Not only does the search converge faster towards well-performing configurations when using TL, it also yields a better configuration on average.
\end{comment}

%%%%%%%% 1-plot version of figure + corresponding text %%%%%%%%
\begin{figure}[t]
    \includegraphics[width=\columnwidth]{img/single-to-full/plot_objective_multi.pdf}
    \caption{Run-time of the best-performing configurations as a function of the search time when adding a workflow step. DeepHyper/PABO workflow uses 128 nodes, each HEP workflow instance uses 4 nodes. The HEP workflow consists of both dataloader and PEP application. We compare the executions with and without TL from results obtained in Section~\ref{sec:Experiments:preliminary}.}
    \label{fig:Experiments:fullwflow}
\end{figure}

Figure~\ref{fig:Experiments:fullwflow} shows the average run-time of the best-performing instances as the search progresses, and the corresponding minimum and maximum.\footnote{The supplemental material provides the corresponding scatter plots for information. These scatter plots do not provide any more relevant information than what is already provided here.} Not only does the search converge faster towards well-performing configurations when using TL, it also yields a better configuration on average. Inspecting the evaluated configurations shows that using TL allows DeepHyper/PABO to start from configurations that are generally better than without TL. This gives an advantage to the TL experiments very early on as instances are able to complete faster, leading to more evaluations, hence better configurations found.

\begin{framed}
By using TL when going from the partial, one-step workflow, to the full workflow, we can achieve an expected search speedup $E(S)$ of $2.85\times$ and improvement factor $F(S)$ of $1.07\times$ for this HEP workflow.
\end{framed}

\subsection{Adding new parameters}
\label{sec:Experiments:newparams}

The experiments in this section aim to show that we can also incrementally add new parameters to our parameter space, and leverage TL to speed up the search for a new well-performing configuration.

We add the last 3 parameters of Table~\ref{tab:parameters}. These parameters tune specific optimizations in the dataloader (the use of a pool of threads to asynchronously process and store data to HEPnOS while the next HDF5 file is being read) and in the PEP application (the use of a prefetcher that loads products in batches in the background so they are readily-available when the processing function needs them). Hence this experiment is also a good example of how to react to the addition of new optimizations that now have to be tuned.

When using TL, we use results from the first repetition of the experiment run in Section~\ref{sec:Experiments:fullwflow} with TL enabled (hence actually chaining transfer-learning results).

\begin{comment}
\begin{figure}[t!]
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/new-parameters/plot_scatter_multi.pdf}
        \caption{Run-time of full workflow instances evaluated by DeepHyper/PABO as the search workflow progresses.}
        \label{fig:Experiments:newparams:a}
    \end{subfigure}
    \par\bigskip
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/new-parameters/plot_objective_multi.pdf}
        \caption{Run-time of the corresponding best-performing configurations as a function of the search time.}
        \label{fig:Experiments:newparams:b}
    \end{subfigure}
    \caption{Adding new parameters: all 19 parameters are used. The DeepHyper/PABO workflow uses 128 nodes; each HEP workflow instance uses 4 nodes. We compare the results with and without TL from results obtained in Section~\ref{sec:Experiments:fullwflow}.}
    \label{fig:Experiments:newparams}
\end{figure}

%Once again DeepHyper/PABO runs for one hour on 128 nodes.
Figure~\ref{fig:Experiments:newparams:a} shows the run time of each configuration evaluated by DeepHyper with and without PABO. Figure~\ref{fig:Experiments:newparams:b} shows the corresponding average, minimum, and maximum best run time, across the 5 repetitions. The conclusion is similar to that of adding a full workflow step: TL generally helps DeepHyper/PABO focus on well-performing regions early on, leading to more configurations evaluated and more efficient configurations found.
\end{comment}

%%%% rewrite of the above with a single figure instead of 2
\begin{figure}[t!]
    \includegraphics[width=\columnwidth]{img/new-parameters/plot_objective_multi.pdf}
    \caption{Run-time of the best-performing configurations as a function of the search time when adding new parameters. All 19 parameters are used. The DeepHyper/PABO workflow uses 128 nodes; each HEP workflow instance uses 4 nodes. We compare the results with and without TL from results obtained in Section~\ref{sec:Experiments:fullwflow}.}
    \label{fig:Experiments:newparams}
\end{figure}

Figure~\ref{fig:Experiments:newparams} shows the average, minimum, and maximum best run time, across the 5 repetitions when executing the search with and without TL. The conclusion is similar to that of adding a full workflow step: TL generally helps DeepHyper/PABO focus on well-performing regions early on, leading to more configurations evaluated and more efficient configurations found.

The minimum and maximum in this figure however show that, while the search without TL achieved worse-performing configurations on average than when using TL, at least one of the runs without TL found a better configuration than with TL, hinting at the possibility that TL overfits its model and focuses too much on regions it knows perform well already, rather than exploring new regions.

\begin{framed}
By using TL when adding new parameters, we can achieve an expected search speedup $E(S)$ of $7.66\times$ and improvement factor $E(F)$ of $1.27\times$ for this workflow.
\end{framed}

We note a better search speedup and improvement factor here than when adding a full workflow step. This is understandable since adding a full workflow step changed the objective function to optimize in addition to adding new parameters. The present scenario simply added three parameters for DeepHyper/PABO to tune.

\subsection{Scaling up workflow instances}
\label{sec:Experiments:scaleup}

Having run the HEP workflow on 4 nodes, we now scale up to 8 then 16 nodes. We use the full workflow with the complete list of 19 parameters. For each scale, we compare the results with and without TL from the 4-node workflow experiments obtained in Section~\ref{sec:Experiments:newparams}.

%We scale accordingly the number of files processed, using 100 files when running instances on 8 nodes, and 200 when running them on 16 nodes.

\begin{comment}
\begin{figure}[t!]
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/scaling-up-8/plot_scatter_multi.pdf}
        \caption{Run-time of full workflow instances evaluated by DeepHyper/PABO as the search workflow progresses.}
        \label{fig:Experiments:scale8:a}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/scaling-up-8/plot_objective_multi.pdf}
        \caption{Run-time of the corresponding best-performing configurations as a function of the search time.}
        \label{fig:Experiments:scale8:b}
    \end{subfigure}
    \caption{Scaling up to 8-node HEP workflow instances. DeepHyper/PABO uses 128 nodes. The full set of parameters is searched, with and without TL from 4-node results obtained in Section~\ref{sec:Experiments:newparams}.}
    \label{fig:Experiments:scale8}
\end{figure}

\begin{figure}[t!]
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/scaling-up-16/plot_scatter_multi.pdf}
        \caption{Run-time of full workflow instances evaluated by DeepHyper/PABO as the search workflow progresses.}
        \label{fig:Experiments:scale16:a}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/scaling-up-16/plot_objective_multi.pdf}
        \caption{Run-time of the corresponding best-performing configurations as a function of the search time.}
        \label{fig:Experiments:scale16:b}
    \end{subfigure}
    \caption{Scaling up to 16-node HEP workflow instances. DeepHyper/PABO uses 128 nodes. The full set of parameters is searched, with and without TL from 4-node results obtained in Section~\ref{sec:Experiments:newparams}.}
    \label{fig:Experiments:scale16}
\end{figure}
\end{comment}

\begin{figure}[t!]
        \includegraphics[width=\columnwidth]{img/scaling-up-8/plot_objective_multi.pdf}
    \caption{Run-time of the best-performing configurations as a function of the search time when scaling up to 8-node HEP workflow instances. DeepHyper/PABO uses 128 nodes. The full set of parameters is searched, with and without TL from 4-node results obtained in Section~\ref{sec:Experiments:newparams}.}
    \label{fig:Experiments:scale8}
\end{figure}

\begin{figure}[t!]
        \includegraphics[width=\columnwidth]{img/scaling-up-16/plot_objective_multi.pdf}
    \caption{Run-time of the best-performing configurations as a function of the search time when scaling up to 16-node HEP workflow instances. DeepHyper/PABO uses 128 nodes. The full set of parameters is searched, with and without TL from 4-node results obtained in Section~\ref{sec:Experiments:newparams}.}
    \label{fig:Experiments:scale16}
\end{figure}

Figure~\ref{fig:Experiments:scale8} and \ref{fig:Experiments:scale16} show once again that TL makes DeepHyper/PABO evaluate more configurations, that are generally more efficient.

TL becomes especially important in this experiment since scaling up each individual HEP workflow instance while keeping the total amount of resources constant means reducing the number of instances that can be evaluated in parallel. While DeepHyper/PABO running on 128 nodes can evaluate 32 4-node configurations at the same time, this number is reduced to 8 when evaluating 16-node configurations. Evaluating poorly-performing configurations due to a lack of prior knowledge slows down the search process dramatically, and greatly reduces the number of configurations that DeepHyper/PABO is able to evaluate within its allotted time. 

\begin{framed}
By using TL when scaling up, we can achieve an expected search speedup $E(S)$ of $8.51\times$ and improvement factor $E(F)$ of $1.23\times$ when going from 4 to 8 nodes, and an expected search speedup $E(S)$ of $10.57\times$ and improvement factor $E(F)$ of $1.84\times$ when scaling from 4 to 16 nodes.
\end{framed}

Although the best-performing configurations at each scale are not exactly the same, the performance of transfer-learning here can be explained by the high correlation that exists between the run time of each configuration at different scales.
 
\subsection{Moving to a new platform}
\label{sec:Experiments:bebop}
 
Lastly, we evaluate whether TL is effective when moving the workflow to a new platform. To stress TL as much as possible, we use a platform vastly different from MachineA: %Argonne's Bebop supercomputer\cite{Bebop},
MachineB, which features Intel Broadwell processors with 36 cores per node, 28GB DDR4 RAM, interconnected via an Intel Omni-Path fabric.

We run DeepHyper/PABO on 128 nodes for an hour, evaluating full-workflow instances on 4 nodes (as in Section~\ref{sec:Experiments:fullwflow}). We use TL from the matching MachineA experiments.

Figure~\ref{fig:Experiments:bebop} shows that, this time, TL does not seem to have much advantage. On average, the final best run-time is similar (30.4 sec without TL, vs. 30.8 sec with TL). The best run time overall (21 sec) is achieved without TL. Still, due to TL converging faster, the expected speedup and improvement factors, respectively 1.45 and 1.10, remain in favor of using TL.

When looking into the configurations explored by DeepHyper/PABO, we note that setting the \texttt{BusySpin} parameter to \texttt{True} seemed particularly important on MachineA. Hence even though MachineB uses a different network, out of 657 evaluations using TL DeepHyper/PABO set this parameter to \texttt{False} only 44 times. The best configurations found without TL showed that it should have been set to \texttt{False} for best performance. This hints at a possible improvement where user knowledge could be combined with autotuning to avoid using a prior on parameters that are likely to change across use-cases.

\begin{comment}
\begin{figure}[t!]
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/bebop/plot_scatter_multi.pdf}
        \caption{Run-time of workflow instances evaluated by DeepHyper/PABO as the search workflow progresses.}
        \label{fig:Experiments:bebop:a}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\columnwidth]{img/bebop/plot_objective_multi.pdf}
        \caption{Run-time of the corresponding best-performing configurations as a function of the search time.}
        \label{fig:Experiments:bebop:b}
    \end{subfigure}
    \caption{Moving the workflow to the MachineB supercomputer, with and without TL from matching MachineA results.}
    \label{fig:Experiments:bebop}
\end{figure}
\end{comment}

\begin{figure}[t!]
        \includegraphics[width=\columnwidth]{img/bebop/plot_objective_multi.pdf}
    \caption{Run-time of the best-performing configurations as a function of the search time when moving the workflow to the MachineB supercomputer, with and without TL from matching MachineA results.}
    \label{fig:Experiments:bebop}
\end{figure}

\begin{framed}
TL is less effective when moving to a radically different platform, in particular when parameters are involved that have no reason to influence performance in the same manner across platforms. TL still remains better in terms of expected speedup and improvement factor.
\end{framed}

\subsection{Synthesis of our results}
 
Table~\ref{tab:summary} summarizes the experiments presented above. The use of TL appears overwhelmingly beneficial to both the search time and the expected improvement factor in all the scenarios except when moving to a new platform, where results are comparable to those obtained without TL.

\begin{table*}[]
\centering
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|}
\cline{2-13}
 & \multicolumn{5}{c|}{\textbf{Without transfer-learning}} & \multicolumn{7}{c|}{\textbf{With transfer-learning}} \\ \cline{1-1}
\multicolumn{1}{|l|}{Sec.} & \textbf{Eval.} & \textbf{T.out} & \textbf{Fail.} & \textbf{Best} & \textbf{Best (avg)} & \textbf{Eval.} & \textbf{T.out} & \textbf{Fail.} & \textbf{Best} & \textbf{Best (avg)} & \textbf{E(S)} & \textbf{E(F)} \\ \hline
\multicolumn{1}{|l|}{\textbf{\ref{sec:Experiments:preliminary}}} & 2500 & 158 & 6 & 9 sec & 9 sec & N/A & N/A & N/A & N/A & N/A & N/A & N/A \\ \hline
\multicolumn{1}{|l|}{\textbf{\ref{sec:Experiments:fullwflow}}} & 1205 & 309 & 19 & 32 sec & 34.4 sec & 1143 & 295 & 22 & \textbf{30 sec} & \textbf{32.6 sec} & \textbf{2.86} & \textbf{1.07} \\ \hline
\multicolumn{1}{|l|}{\textbf{\ref{sec:Experiments:newparams}}} & 746 & 247 & 17 & \textbf{28 sec} & 35.8 sec & 1056 & 288 & 17 & 29 sec & \textbf{30.2 sec} & \textbf{7.66} & \textbf{1.27} \\ \hline
\multicolumn{1}{|l|}{\textbf{\ref{sec:Experiments:scaleup} (8)}} & 513 & 176 & 5 & \textbf{35 sec} & 42.4 sec & 548 & 174 & 2 & 37 sec & \textbf{38.6 sec} & \textbf{8.51} & \textbf{1.23} \\ \hline
\multicolumn{1}{|l|}{\textbf{\ref{sec:Experiments:scaleup} (16)}} & 208 & 84 & 2 & 47 sec & 71.8 sec & 254 & 85 & 0 & \textbf{41 sec} & \textbf{44.4 sec} & \textbf{10.57} & \textbf{1.84} \\ \hline
\multicolumn{1}{|l|}{\textbf{\ref{sec:Experiments:bebop}}} & 562 & 291 & 36 & \textbf{21 sec} & \textbf{30.4 sec} & 657 & 278 & 46 & 27 sec & 30.8 sec & \textbf{1.45} & \textbf{1.10} \\ \hline
\end{tabular}
\caption{Summary of the experiments done in this paper. \textit{Eval.} = total number of configurations evaluated across 5 searches, on 128 nodes, for 1 hour. \textit{T.out} = number of evaluations that timed out. \textit{Fail.} = number of evaluations that failed. \textit{Best} = run time of the best configuration found across all 5 searches. \textit{Best (avg)} = average best run time across all 5 searches.}\label{tab:summary}
\end{table*}

==> sections/old/Motivation.tex <==
Since 2018, the SciDAC ``HEP-on-HPC''~\cite{HEPonHPC} project has brought together physicists and computer scientists from a number of institutions around the challenges of leveraging HPC resources to solve large-scale HEP problems. One outcome of this project was HEPnOS, a storage service designed by Argonne National Laboratory to store and provide access to billions of ``event'' data produced by particle accelerators. HEPnOS serves as a centerpiece for a number of HEP analytic workflows, one of which is the event-selection workflow~\cite{paterno2019parallel} for the NOvA experiment~\cite{NOvApaper, NOvA}.

As a highly configurable data service, HEPnOS offers ways to be finely tuned for specific use-cases. However finding an optimal configuration for a particular application on a particular platform remains a challenge. Researchers at Argonne and FermiLab have spent the past couple of years trying to understand how each parameter influences performance, relying on trial-and-error, manual tuning, benchmarking, and profiling. In this paper we aim to automatize this tuning process by using parameter-space exploration and Bayesian optimization. This section dives into the technical details of HEPnOS and the event-selection workflow that are relevant to our endeavour. 

% -----------------------------------------------------------------
% -----------------------------------------------------------------
\subsection{The HEPnOS storage system}
\label{sec:Motivation:hepnos}

HEPnOS was designed to store HEP data in a hierarchy of \emph{datasets}, \emph{runs}, \emph{subruns}, \emph{events}, and \emph{products}. Datasets are named-containers of runs. Runs, subruns, and events are identified by numbers. Events are containers for products, which are vectors of C++ objects ranging from a few bytes to a few KB and identified by their type and a user-provided label. On servers, HEPnOS organizes this hierarchy in a collection of flat key/value stores, providing a \texttt{put/get} interface for products, and iteration capabilities over datasets, runs, subruns, and events.

\subsection{HEPnOS' software overview}
\label{sec:Motivation:hepnos:overview}

HEPnOS was built using components from the Mochi project~\cite{ross2020mochi}, which advocates for the development of reusable, interoperable building blocks in the design of HPC data services. Mochi services in general, and HEPnOS in particular, rely on Mercury~\cite{soumagne2013mercury} for remote procedure calls (RPC) and remote direct memory access (RDMA), and on Argobots~\cite{seo2017argobots} for thread management. The Margo~\cite{Margo} library binds Mercury and Argobots together to provide a simple abstraction for developing remotely-accessible microservices. Different microservices (or ``providers'') can live in the same process and share the same threading runtime and network progress loop thanks to Margo.

On top of Margo, HEPnOS uses the SDSKV microservice~\cite{SDSKV} to provide key/value storage capabilities, and the Bedrock microservice~\cite{Bedrock} to provide bootstrapping and configuration capabilities. This architecture is shown in Figure~\ref{fig:hepnos}.

% All the diagrams are at the following address:
% https://drive.google.com/file/d/1apuAz9io6MjTGUAG98BITmyWGsirSesD/view?usp=sharing

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{5.6cm}
        \includegraphics[width=5.6cm]{img/HEPnOS.pdf}
        \caption{HEPnOS}
        \label{fig:hepnos}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{5.6cm}
        \includegraphics[width=5.6cm]{img/DataLoader.pdf}
        \caption{Data loader}
        \label{fig:dataloader}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{5.6cm}
        \includegraphics[width=5.6cm]{img/EventSelection.pdf}
        \caption{Event selection}
        \label{fig:eventselection}
    \end{subfigure}
    \caption{Overview of the HEP workflow and HEPnOS storage system. A set of HDF5 files containing tables of event data is read by a parallel application, the Dataloader, which converts them into arrays of C++ objects that are then stored in HEPnOS. In the Event-selection step, all the events contained in a given \emph{run} are read and processed in parallel to search for events matching specific criterion.}
    \label{fig:Motivation:schemas}
\end{figure*}

\subsubsection{Key/value storage and organization in HEPnOS}
\label{sec:Motivation:hepnos:organization}

%\RE{maybe try to clarify a bit. I found confusing the changed order of subrun/run/dataset with respect to dataset/run/subrun in the intro of the section}

Each HEPnOS server manages a set of key/value databases, used to store events, and another set of databases to store products. The number of databases storing events may be different from the number of databases storing products. Both numbers are configurable.

Each event is referenced by a key in the form \texttt{<dataset id, run number, subrun number, event number>}. The database instance storing each such key is selected via consistent hashing of its \texttt{<dataset id, run number, subrun number>} part. Hence all the events belonging to the same dataset/run/subrun hierarchy end up in the same database. Products are identified by a similar key, with the addition of two extra fields (type and label), and are hashed the same way as events, using only their dataset id, run number, and subrun number.

This data distribution ensures that iterating over events and products in a specific subrun -- a common pattern in HEP workflows -- can be done by interacting with only two database instances (one for events and one for products) and can be optimized using batching and prefetching strategies.

\subsubsection{Configuring and bootstrapping HEPnOS}
\label{sec:Motivation:hepnos:configuration}

Thanks to the Bedrock component, which provides configuration and bootstrapping capabilities to Mochi microservices, HEPnOS is configured via a JSON file that describes which components need to be dynamically loaded, and how they should be configured. Based on this file, Bedrock bootstraps the networking component (Mercury), the threading component (Argobots) and the key/value storage component (SDSKV).

This extensive configurability is critical to the work presented in this paper. It allows us to finely tune every single aspect of the service, from high-level parameters of the key/value storage component (such as how many databases to manage on each node), to how threading is performed (number of threads, scheduling policies, assignment of threads to databases), down to details of the networking layer such as whether to use blocking \texttt{epoll} or busy-spinning.

% -----------------------------------------------------------------
% -----------------------------------------------------------------
\subsection{The NOvA event-selection workflow}
\label{sec:Motivation:workflow}

HEPnOS is used as temporary, distributed, in-memory storage system for HEP workflows. In this work we focus on the NOvA event-selection workflow, which consists of two steps: data-loading, and parallel-event-processing.

%
% DATA LOADING
%
\subsubsection{Data loading}
\label{sec:Motivation:workflow:dataloader}

In practice, the event-selection workflow does not operate directly on data as it is produced by the particle accelerator. The raw data is first stored into files, either in HDF5~\cite{hdf5} or in ROOT~\cite{ROOT} format. While these files can be shared across institutions easily, they produce an I/O bottleneck when it comes to reading them. Hence in HEPnOS-based workflows they need to be loaded into HEPnOS prior to being analyzed.

The dataloader, shown in Figure~\ref{fig:dataloader}, is in charge of this task. It is a parallel, MPI-based application that takes as input a list of HDF5 files, and converts them back into C++ objects that are then stored in HEPnOS. Each HDF5 file contains all the products for all the events of a single subrun. Hence given the data organization explained in Section~\ref{sec:Motivation:hepnos:organization}, all the data stored in an HDF5 file will end up in a couple of databases: one for its events, and one for its products.

Since the amount of data differs across HDF5 files, the dataloader does not distribute the work in a static manner across its processes. Instead, a list of files is maintained in one process, and all the processes pull work from this shared list of files, until all the files have been loaded.

Several optimizations are available in the dataloader, including batching data prior to storage into HEPnOS (reducing the number of RPCs and increasing the payload of RDMA operations), and overlapping the loading/conversion of a file with the storage of data from a previous file into HEPnOS. These optimizations can be turned on or off and configured in various ways. Along with job-related parameters (number processes, number of threads, mapping to CPUs), the dataloader offers many configurations parameters that can be tuned to achieve good performance.

%
% PARALLEL EVENT PROCESSING
%
\subsubsection{Parallel event processing}
\label{sec:Motivation:workflow:pep}

The second step of the workflow, \emph{parallel event processing} (PEP), shown in Figure~\ref{fig:eventselection}, consists of reading the events and some products of interest from HEPnOS, and performing some computation on the data to determine events of interests.%\footnote{The reader may wonder why this step is not performed from the HDF5 files directly, and why HEPnOS is needed at all. The reason is that the workflow presented in this paper represents a subset of larger workflows involving more steps before and after the two presented here. For example the data read from HEPnOS in the event-selection step may have been produced by a simulation of the particle accelerator, rather than coming from HDF5 files, and the event-selection step could be replaced with other steps that load and store data, most of which is temporary and is more efficiently accessed via HEPnOS.}

Assuming events are stored in $N$ databases in HEPnOS, $N$ processes of the PEP application are used to list them, each from one database.%\footnote{If the PEP application runs on fewer than $N$ processes, each process may read from multiple databases}
%
They end up with a local list of keys \texttt{<dataset id, run number, subrun, number event number>}, where \texttt{dataset id} is a UUID uniquely representing the dataset that is being read, and \texttt{run}, \texttt{subrun}, and \texttt{event numbers} are 64-bit identifiers. All the processes then process events by pulling these keys from their local queue or by requesting batches of keys from other processes if their local queue is empty.

Events are processed first by loading the data products associated with them, then by computing on these products. The PEP application provides a benchmark of its I/O part (loading events and products) that simulates computations rather than actually performing them. We use this benchmark in place of the PEP application in this paper since the actual application is much more complex to build and run.

Just like HEPnOS and the dataloader, optimizations are in place to improve I/O performance in the PEP application and benchmark: look-ahead prefetching when reading from HEPnOS, batching of event keys when they are loaded and when they are sent from a process to another, batching of data products, and multithreaded processing of events inside each process. All these optimizations come with their own set of tunable parameters that can influence the overall performance of the workflow.

%
% CHALLENGES
%
\subsection{Challenges of (auto)tuning the workflow}

While the parameters of a single workflow component cannot be tuned independently from one another, they also cannot be tuned independently from that of other components. As an example, what could seem like an optimal number of threads in the PEP application could in turn influence the optimal number of databases in HEPnOS, which could influence the batch size used by the dataloader when storing events into HEPnOS. Manually tuning such a workflow becomes rapidly intractable, in particular as new optimizations (hence new parameters) are implemented, new steps are added to the workflow, when the workflow scales up, or when it is ported to a new platform. This motivated us to investigate ways of automatically tuning such a workflow using parameter space exploration and machine learning.% \RE{can be refered as "derivative free" optimisation or black-box optimisation}.

Parameter-space exploration enables defining the list of tunable parameters and their domain. It then uses a ``meta-workflow'' to execute multiple instances of the workflow in parallel, with different configurations, in order to measure how fast they complete when given a relatively small number of HDF5 files as input. This method however poses an important challenge: evaluating many configurations consumes a lot of computation resources, especially as the parameter space grows and as the use-case gets more complex. %\RE{but we always used 128 nodes on Theta? I understand the argument about the speed-up but maybe this needs to be formulated differently}
Hence, this paper focuses on ways to speed up such an exploration process by (1) using a surrogate model to approximate the workflow performance as a function of its configuration, and (2) using transfer learning to go from a small-scale, one-step workflow with few parameters, to a large-scale, full workflow with more parameters. The next section presents these two contributions. %The parameters we consider for each component of the workflow are listed in Table~\ref{tab:parameters}.
